IGLUE: A Benchmark for Transfer Learning across Modalities, Tasks, and Languages

Reliable evaluation benchmarks designed for replicability and comprehensiveness have driven progress in machine learning. Due to the lack of a multilingual benchmark, however, vision-and-language research has mostly focused on English language tasks. To fill this gap, we introduce the Image-Grounded Language Understanding Evaluation benchmark. IGLUE brings together - by both aggregating pre-existing datasets and creating new ones - visual question answering, cross-modal retrieval, grounded reasoning, and grounded entailment tasks across 20 diverse languages. Our benchmark enables the evaluation of multilingual multimodal models for transfer learning, not only in a zero-shot setting, but also in newly defined few-shot learning setups. Based on the evaluation of the available state-of-the-art models, we find that translate-test transfer is superior to zero-shot transfer and that few-shot learning is hard to harness for many tasks. Moreover, downstream performance is partially explained by the amount of available unlabelled textual data for pretraining, and only weakly by the typological distance of target-source languages. We hope to encourage future research efforts in this area by releasing the benchmark to the community.

==> 06_analysis.tex <==
% We now provide a series of further and finer-grained analyses, which include: additional comparisons with the `translate train' transfer approach (\S\ref{sec:compare_trans_train}), the analysis of performance over structurally different question types of xGQA in few-shot setups (\S\ref{sec:struc_analys_xgqa}) and domain-specific retrieval results in xFlickr\&CO (\S\ref{sec:perf_eval_subset}). 


% \begin{figure*}[t]
%  	\centering
%  	\includegraphics[width=\linewidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/xGQA_Struct_FewShot.pdf}%
%  	\caption{Analysis of few-shot results on xGQA over 5 structurally different questions types; see also \cite{pfeiffer2021xgqa} for further details on the question types.}
%  	\label{fig:fewshot-xgqa-struct}
% \end{figure*}


% \begin{table}[t]
% \caption{Pearson's coefficients and corresponding p-values (in brackets) between
% dataset- and language-level \emph{cross-lingual performance gap} (English acc - target language acc) and various metrics evaluated across all models. The Pearson's coefficient for the Genetic distance in MaRVL is undefined since each language is at distance 1.0 from English.}
% \label{tab:uriel}
% \vskip 0.15in
% \setlength\tabcolsep{1.5pt}
% \small
% \center
%   \resizebox{0.48\textwidth}{!}{
% %   \begin{tabular}{lccccccc}
%   \begin{tabular}{lrrrrrr}
% \toprule
% & \multicolumn{1}{c}{\textbf{Genetic}} & \multicolumn{1}{c}{\textbf{Syntactic}} & \multicolumn{1}{c}{\textbf{Featural}} & \multicolumn{1}{c}{\textbf{Phonological}} & \multicolumn{1}{c}{\textbf{Inventory}} & \multicolumn{1}{c}{\textbf{Geographic}} \\
% % \multirow{2}{*}{\small \shortstack{\textbf{Model}}}         &  \multicolumn{1}{c}{\textbf{NLI}}   & \multicolumn{1}{c}{\textbf{QA}} & \multicolumn{1}{c}{\textbf{Reasoning}}  & \multicolumn{4}{c}{\textbf{Retrieval}} \\
% %   \cmidrule(r){2-2}
% %   \cmidrule(r){3-3}
% %   \cmidrule(r){4-4}
% %   \cmidrule(r){5-8}
% %  & \multicolumn{1}{c}{XVNLI} & \multicolumn{1}{c}{xGQA}     & \multicolumn{1}{c}{MaRVL} & \multicolumn{2}{c}{xFlickr\&CO}          & \multicolumn{2}{c}{WIT}        \\
% \midrule
% \emph{Dataset} & \multicolumn{6}{c}{} \\
% \midrule
% XVNLI & 0.60 (0.014) & 0.52 (0.039) & 0.60 (0.014) & 0.44 (0.088) & 0.58 (0.017) & 0.45 (0.078) \\
% xGQA & 0.40 (0.033) & 0.55 (0.002) & 0.46 (0.014) & 0.18 (0.348) & 0.25 (0.197) & 0.25 (0.199) \\
% MaRVL & nan (nan) & -0.07 (0.774) & 0.06 (0.791) & 0.19 (0.425) & 0.15 (0.521) & 0.25 (0.291) \\
% xFlickr\&CO & 0.17 (0.398) & 0.27 (0.168) & 0.15 (0.438) & -0.01 (0.943) & -0.06 (0.762) & -0.04 (0.837) \\
% WIT & 0.29 (0.066) & 0.25 (0.114) & 0.19 (0.248) & 0.29 (0.072) & 0.19 (0.236) & -0.09 (0.599) \\
% \midrule
% \emph{Language} & \multicolumn{6}{c}{} \\
% \midrule
% ARB & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% BEN & 0.34 (0.03) & 0.30 (0.06) & 0.22 (0.17) & 0.34 (0.03) & 0.23 (0.16) & -0.10 (0.54) \\
% BUL & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% DAN & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% EST & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% DEU & 0.14 (0.38) & 0.12 (0.45) & 0.09 (0.58) & 0.14 (0.39) & 0.09 (0.56) & -0.04 (0.80) \\
% ELL & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% FRA & 0.34 (0.03) & 0.30 (0.06) & 0.22 (0.18) & 0.34 (0.03) & 0.22 (0.16) & -0.10 (0.54) \\
% IND & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% JPN & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% KOR & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% CMN & 0.14 (0.38) & 0.12 (0.45) & 0.09 (0.58) & 0.14 (0.39) & 0.09 (0.56) & -0.04 (0.80) \\
% POR & 0.34 (0.03) & 0.30 (0.06) & 0.22 (0.17) & 0.34 (0.03) & 0.23 (0.16) & -0.10 (0.54) \\
% RUS & 0.14 (0.38) & 0.12 (0.45) & 0.09 (0.58) & 0.14 (0.39) & 0.09 (0.56) & -0.04 (0.80) \\
% SPA & 0.14 (0.38) & 0.12 (0.45) & 0.09 (0.58) & 0.14 (0.39) & 0.09 (0.56) & -0.04 (0.80) \\
% SWA & 0.31 (0.05) & 0.27 (0.09) & 0.20 (0.22) & 0.31 (0.05) & 0.20 (0.21) & -0.09 (0.58) \\
% TAM & 0.31 (0.05) & 0.27 (0.09) & 0.20 (0.22) & 0.31 (0.05) & 0.20 (0.21) & -0.09 (0.58) \\
% TUR & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% VIE & 0.29 (0.07) & 0.25 (0.11) & 0.19 (0.25) & 0.29 (0.07) & 0.19 (0.24) & -0.09 (0.60) \\
% \bottomrule
% \end{tabular}
% }
% % \caption{Pearson's coefficients and corresponding p-values (in brackets) between
% % dataset- and language-level \emph{cross-lingual performance gap} (english acc - language acc) and various metrics evaluated across all models. The Pearson's coefficient for the Genetic distance in MaRVL is undefined since each language is at distance 1.0 from English. \label{tab:uriel}}
% \end{table}


%More analyses on xFlickr (esp. \german{} and \japanese).

% \rparagraph{Performance with more shots} 
% In the few-shot experiments, we noticed no observable improvement or clear trend of performance increase on 3 our of the 4 tasks. Here we pick the task of retrieval and xFlickr dataset to further understand if it is the number of shots are too few. In \Cref{fig:fewshot-curves-xflickr-deja}, we plot \german{} and \japanese{} performances with up to 1500 shots (instead of the 100 shots used in the few-shot setting).\footnote{\german{} and \japanese{} captions are from Multi30k and \citet{nakayama-etal-2020-visually} respectively.} Indeed, we observe an over trend of performance increase with more number of training examples, however with instability (e.g. for UC$^2$ on \japanese, its performance dropped a little when shots are more than 500).

% \subsection{Comparison with Translate Train} 
% \label{sec:compare_trans_train}
% We further compare the 1{,}500-shot models with `translate-train` models: we directly fine-tune the original UC$^2$ and xUNITER checkpoints with the full xFlickr training set human-translated to \german{} and \japanese{} (the same data source as used in the previous 1500-shot setups, but we now use all the data: 29k images and 145k captions). As shown in \Cref{fig:fewshot-curves-xflickr-deja}, UC$^2$ \footnote{Note that UC$^2$ is pretrained on Conceptual Captions translated also in \german{} and \japanese.} in the 1500-shot transfer setup reaches or surpasses performance of `translate-train', while xUNITER also reaps benefits of the `many-shot' setup,  but it is still far from `translate-train' performance in the same setup (despite being initialised from English fine-tuned weights).

% Further we note that `translate-train' performance is still far from the corresponding English performance -- this is a bit surprising at least for UC$^2$, as the model was pretrained solely on translations of Conceptual Captions, each of the same size.\ivan{Not related to this part, but: 1) Table is not referenced nor referred to anywhere. What does it convey? Do we need a short analysis of it? 2) There are some tables which are never referenced anywhere - we should at least write a one sentence summary of what they contain in the appendix.}
    

% \paragraph{More images or more captions?} An important question concerning data collection efficiency for more languages in text-image retrieval is that, should we collect more captions per image or more images with a single caption? We trained xUNITER and UC$^2$ on \japanese{} and \german{} data with different number of shots and different caption per image ration
% (\Cref{tab:FlickrCO-num-ir}). As results shown in the table, there is no clear trend suggesting one is better than the other. We leave a more large-scale investigation on this for future research. 

% \begin{table}[t]
% \caption{Caption density in xFlickr\&CO.}
% \label{tab:FlickrCO-num-ir}
% \vskip 0.15in
% \setlength\tabcolsep{3pt}
% \small
% \center
%   \resizebox{0.48\textwidth}{!}{
%   \begin{tabular}{rrr|rr|rr|rr|rr}
% \toprule
% \multicolumn{3}{l|}{\textbf{xFlickr\&CO}} & \multicolumn{2}{c|}{\textbf{\german{} IR}} & \multicolumn{2}{c|}{\textbf{\japanese{} IR}} & \multicolumn{2}{c|}{\textbf{\german{} TR}} & \multicolumn{2}{c}{\textbf{\japanese{} TR}} \\
% \textbf{\# shots} & \textbf{\# img} & \textbf{\# cap/img} & \multicolumn{1}{c}{\textbf{xUNI}} & \multicolumn{1}{c|}{\textbf{UC$^2$}} & \multicolumn{1}{c}{\textbf{xUNI}} & \multicolumn{1}{c|}{\textbf{UC$^2$}} & \multicolumn{1}{c}{\textbf{xUNI}} & \multicolumn{1}{c|}{\textbf{UC$^2$}} & \multicolumn{1}{c}{\textbf{xUNI}} & \multicolumn{1}{c}{\textbf{UC$^2$}} \\
% \midrule
% \multirow{2}{*}{\small \shortstack{500}} & 500 & 1 & \textbf{17.15} & 27.20 & 11.95 & \textbf{29.35} & \textbf{14.80} & 21.40 & \textbf{13.05} & \textbf{25.45} \\
% & 100 & 5 & 13.70 & \textbf{30.60} & \textbf{14.00} & 23.60 & 9.80 & \textbf{25.10} & 12.50 & 21.70 \\
% \midrule
% \multirow{2}{*}{\small \shortstack{1000}} & 1000 & 1 & 15.50 & \textbf{30.55} & 12.70 & \textbf{28.90} & 14.20 & \textbf{24.65} & \textbf{12.65} & 26.00 \\
% & 200 & 5 & \textbf{15.85} & 26.30 & \textbf{14.35} & 28.40 & \textbf{14.25} & 20.35 & 12.15 & \textbf{26.30} \\
% \bottomrule
% \end{tabular}
% }
% % \caption{Caption density in xFlickr\&CO. \label{tab:FlickrCO-num-ir}}
% \end{table}

% \subsection{xGQA: Analysis over Question Types}
% \label{sec:struc_analys_xgqa}
% To better understand the impact of few-shot experiments on xGQA, we plot the results grouped by each structurally different question type in Figure~\ref{fig:fewshot-xgqa-struct}. We find that increasing the number of examples has the least impact on \textit{Verify}-type questions, which consist of (binary) answers/labels \textit{\{Yes, No\}}. These results are in line with our few-shot experiments on the other tasks, where few-shot tuning displays negligible impact on cross-lingual transfer performance when the label space is small. The largest impact in few-shot setups is observed on \textit{Choose}-type and \textit{Query}-type questions, where the diversity of the label space is large. This again demonstrates that the multilingual misalignment of the prediction space negatively impacts zero-shot results, which we can mitigate by further fine-tuning even on a handful of examples in the target language. 


% \subsection{MaRVL: Additional Analysis}
% \label{sec:analysis_marvl}
% %\fangyu{I'll write this today or tomorrow!}
% The few-shot results from \Cref{tab:marvl}) demonstrate some modest gains in few-shot setups, but there are no clear trends emerging. In other words, we observe a substantial variation in the reported few-shot results -- performance does not grow steadily and consistently with the number of shots. We also note that xUNITER is the strongest model on \textsc{ind} and \textsc{tur}; on \textsc{cmn} UC$^2$ substantially outperforms all other models. This might be due to UC$^2$ being pre-trained on \textsc{cmn} texts.



% \subsection{Retrieval: Performance by Evaluation Subset}
% \label{sec:perf_eval_subset}
% \begin{table}[t]
% \caption{English image retrieval performance by evaluation subset in xFlickr\&CO after fine-tuning.} 
% \label{tab:FlickrCO-subset}
% \vskip 0.15in
% \setlength\tabcolsep{3pt}
% \small
% \center
% %   \resizebox{0.48\textwidth}{!}{
%   \begin{tabular}{lrrrr}
% \toprule
% \textbf{xFlickr\&CO subset} & \multicolumn{1}{c}{\textbf{mUNITER}} & \multicolumn{1}{c}{\textbf{xUNITER}} & \multicolumn{1}{c}{\textbf{UC$^2$}} & \multicolumn{1}{c}{\textbf{M$^3$P}} \\ 
% \midrule
% Flickr & \textbf{51.3} & \textbf{46.6} & \textbf{44.0} & \textbf{37.1} \\
% COCO & 37.7 & 30.3 & 30.8 & 25.6 \\
% \bottomrule
% \end{tabular}
% % }
% % \caption{English image retrieval performance by evaluation subset in xFlickr\&CO after fine-tuning.} \label{tab:FlickrCO-subset}
% \end{table}

% \begin{figure}[t]
%  	\centering
%  	\includegraphics[width=\linewidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/fewshot_curves_xFlickr-subset.pdf}%
%  	\caption{Image retrieval performance averaged across languages per xFlickr\&CO subset.}
%  	\label{fig:fewshot-curves-xflickr-subset}
% \end{figure}

% \begin{figure}[t]
%  	\centering
%  	\includegraphics[width=\linewidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/fewshot_curves_UC2_xFlickr-subset.pdf}%
%  	\caption{UC$^2$ image retrieval performance across languages per xFlickr\&CO subset.}
%  	\label{fig:fewshot-curves-uc2-xflickr-subset}
% \end{figure}

% Our xFlickr\&CO dataset is a composition of (translated) Flickr and COCO data, which are essentially data of two slightly different domains. Comparing model performances on the Flickr and COCO subsets both in English and in other languages helps us understand if the model behaviour is preserved after zero-shot transfer. If we focus on one model, UC$^2$, as shown in \Cref{tab:FlickrCO-subset},
% its performance on the Flickr subset is higher than on the COCO subset for English.\ivan{I am not fully sure about the argument in the entire subsection; is it sane to compare absolute scores if we don't have equal test subsets in COCO versus Flickr? Can someone take a look?} However, this does not hold true for cross-lingual transfer results -- the absolute scores on COCO is on par or slightly better, both in zero-shot (\Cref{fig:fewshot-curves-uc2-xflickr-subset}) and in few-shot (\Cref{fig:fewshot-curves-xflickr-subset}) settings.
% %This is also true for each individual language as shown in \Cref{} for UC$^2$.
% This shows that models are still learning the task on the target language rather than learning the domain itself (otherwise, the multilingual models would still perform better on Flickr). We foresee domain adaptation as a potential challenge in xFlickr\&CO for future, tightly-multilingual models.
% % If so, few-shot is still working but to solve xFlickr\&CO, models need to generalise across domains.
% \fangyu{Here the arguments are a bit complicated and hard to process. @ema, please check if I interpreted your figures correctly.}


% \iffalse

\subsection{Current Limitations and Future Considerations}
\label{sec:limitations}
(If there's space) List one-paragraph ideas and considerations: 1) how scores on the current benchmark can be improved -- what are the paths going forward? 2) how the current benchmark can be improved and extended. In other words: Discuss what (we think) are still main current limitations of our dataset, and how we plan to enrich it further. However, conclude in positive tones: this will be extremely useful due to X,Y,Z...

- Expand the few-shot setup? (i.e. more shots)
\fi

%\fangyu{merge with conclusion?}



